UNIK: A Unified Framework for Real-world Skeleton-based Action Recognition

Action recognition based on skeleton data has recently witnessed increasing attention and progress. State-of-the-art approaches adopting Graph Convolutional networks (GCNs) can effectively extract features on human skeletons relying on the pre-defined human topology. Despite associated progress, GCN-based methods have difficulties to generalize across domains, especially with different human topological structures. In this context, we introduce UNIK, a novel skeleton-based action recognition method that is not only effective to learn spatio-temporal features on human skeleton sequences but also able to generalize across datasets. This is achieved by learning an optimal dependency matrix from the uniform distribution based on a multi-head attention mechanism. Subsequently, to study the cross-domain generalizability of skeleton-based action recognition in real-world videos, we re-evaluate state-of-the-art approaches as well as the proposed UNIK in light of a novel Posetics dataset. This dataset is created from Kinetics-400 videos by estimating, refining and filtering poses. We provide an analysis on how much performance improves on smaller benchmark datasets after pre-training on Posetics for the action classification task. Experimental results show that the proposed UNIK, with pre-training on Posetics, generalizes well and outperforms state-of-the-art when transferred onto four target action classification datasets: Toyota Smarthome, Penn Action, NTU-RGB+D 60 and NTU-RGB+D 120.

==> tables/ntu-120.tex <==
\begin{table}[t]
\centering

\begin{center}
\scalebox{0.85}{
%2.0
\setlength{\tabcolsep}{3.0mm}{
\begin{tabular}{ l c c c }
\hline
\multirow{2}*{\textbf{Methods}} &\multicolumn{2}{c}{\textbf{NTU-RGB+D 120}}\\
&\text{CS(\%)} &\text{CSet(\%)} \\
\hline
\hline

2s-AGCN~\cite{2sagcn2019cvpr} &82.9& 84.9\\
%MS-AAGCN~\cite{shi_skeleton-based_2019}&&\\
MS-G3D Net~\cite{liu2020disentangling} &\text{86.9} &\text{88.4}\\

\hline
ST-LSTM~\cite{ST-LSTM} & 55.7 & 57.9\\
GCA-LSTM~\cite{GCA-LSTM} & 61.2 & 63.3\\
RotClips + MTCNN~\cite{Clip-2018} & 62.2 & 61.8\\
Body Pose Evolution Map~\cite{Maps-2018} & 64.6 & 66.9\\

\hline
\text{UNIK w/o pt. (Ours)} &\text{83.6} &\text{85.5} \\
MS-G3D Net pt. on Posetics (Ours) &\textbf{87.1} &\textbf{88.8}\\
\textbf{UNIK pt. on Posetics (Ours)} &\text{85.0} &\text{86.5} \\
\hline

\end{tabular}}}

\end{center}
\vspace{-0.3cm}
\caption{Classification accuracy comparison with state-of-the-art methods on the NTU-120 Skeleton dataset.}
\vspace{-0.1cm}
\label{tab_ntu12}
\end{table}  

==> tables/ntu-60.tex <==
\begin{table}[t]
\centering

\begin{center}
\scalebox{0.85}{
\setlength{\tabcolsep}{3.0mm}{
\begin{tabular}{ l c c c }
\hline
\multirow{2}*{\textbf{Methods}} &\multicolumn{2}{c}{\textbf{NTU-RGB+D 60}}\\
&\text{CS(\%)} &\text{CV(\%)} \\
\hline
\hline

ST-GCN~\cite{Yan2018SpatialTG}& 81.5& 88.3\\
ST-GR~\cite{Li2019SpatioTemporalGR}&86.9& 92.3\\
AS-GCN~\cite{Li_2019_CVPR} &86.8& 94.2\\
2s-AGCN~\cite{2sagcn2019cvpr} &88.5& 95.1\\
AGC-LSTM~\cite{Si_2019_CVPR} & 89.2 &95.0\\
DGNN~\cite{Shi2019SkeletonBasedAR} &89.9 &96.1 \\
GCN-NAS~\cite{Peng2020LearningGC} &89.4 &95.7\\
MS-AAGCN~\cite{shi_skeleton-based_2019}&\text{90.0} &\text{96.2}\\
MS-G3D Net~\cite{liu2020disentangling}&\text{91.5} &\text{96.2}\\

%2s MST-GCN (AAAI 21) 96.4 91.1
\hline
IndRNN~\cite{Li2018IndependentlyRN}&81.8& 88.0\\
HCN~\cite{Li2018CooccurrenceFL}&86.5& 91.1\\
VA-fusion~\cite{zhang2019view}&89.4&95.0\\
\hline
\text{UNIK w/o pt. (Ours)} &\text{89.5} &\text{95.7} \\
MS-G3D Net pt. on Posetics (Ours) &\textbf{91.7} &\text{96.2}\\
\textbf{UNIK pt. on Posetics (Ours)} &\text{89.7} &\textbf{96.4} \\
\hline

\end{tabular}}}
\end{center}
\vspace{-0.3cm}
\caption{Classification accuracy comparison with state-of-the-art methods on the NTU-60 Skeleton dataset.}
\vspace{-0.1cm}
\label{tab_ntu60}
\end{table}  

==> tables/posetics.tex <==

\begin{table}[t]
\centering
\begin{center}
\scalebox{0.62}{

%\setlength{\tabcolsep}{1.1mm}{
\begin{tabular}{ l c c }
\hline
\multirow{2}*{\textbf{Methods}}  & \multicolumn{2}{c}{\textbf{Posetics}} \\

& \text{Top-1(\%)} &\text{Top-5(\%)} \\
\hline
\hline
TCNs~\cite{tcn} & 34.0 &57.2\\
%ST-GCN~\cite{Yan2018SpatialTG}&& 2D skeletons, graph $Adj$ &43.3 &67.3\\
ST-GCN~\cite{Yan2018SpatialTG}  &43.3 &67.3\\


2s-AGCN~\cite{2sagcn2019cvpr}  &47.0 &70.8 \\
MS-G3D Net~\cite{liu2020disentangling}  &47.1 &70.0 \\
\hline
%ST-LDN-OpenPose~\cite{OpenPose}&& 45.9 & 69.5\\
\textbf{UNIK (Ours)} &\textbf{47.6} &\textbf{71.3} \\


\hline
\end{tabular}}
%}}
\end{center}
\vspace{-0.3cm}
\caption{Classification accuracy of baselines and the proposed method on the Posetics dataset.}
\vspace{-0.4cm}
\label{tab_posetics}
\end{table}  

